API Usage Recommendation via Multi-View Heterogeneous Graph Representation Learning

Developers often need to decide which APIs to use for the functions being implemented. With the ever-growing number of APIs and libraries, it becomes increasingly difficult for developers to find appropriate APIs, indicating the necessity of automatic API usage recommendation. Previous studies adopt statistical models or collaborative filtering methods to mine the implicit API usage patterns for recommendation. However, they rely on the occurrence frequencies of APIs for mining usage patterns, thus prone to fail for the low-frequency APIs. Besides, prior studies generally regard the API call interaction graph as homogeneous graph, ignoring the rich information (e.g., edge types) in the structure graph. In this work, we propose a novel method named MEGA for improving the recommendation accuracy especially for the low-frequency APIs. Specifically, besides call interaction graph, MEGA considers another two new heterogeneous graphs: global API co-occurrence graph enriched with the API frequency information and hierarchical structure graph enriched with the project component information. With the three multi-view heterogeneous graphs, MEGA can capture the API usage patterns more accurately. Experiments on three Java benchmark datasets demonstrate that MEGA significantly outperforms the baseline models by at least 19% with respect to the Success Rate@1 metric. Especially, for the low-frequency APIs, MEGA also increases the baselines by at least 55% regarding the Success Rate@1.

==> sections/formulation.tex <==


In this section, we first introduce four types of graph, i.e.,\emph{call interaction graph, API global co-occurrence graph, method hierarchical relation graph, and API hierarchical relation graph}, and then present the task description.

Following the formulation of mainstream recommendation systems, we treat all the method declarations in projects as user set ${\mathcal{U}}$, and all the APIs invocated by methods as item set $\mathcal{I}$.

\noindent\textbf{Call Interaction Graph:} In an API recommendation scenario, there exists call relations between method and API. Here we represent these interaction data as a bipartite graph \\
${\mathcal{G}_I=\{(u,y_{ui},i)| u\in\mathcal{U},i\in\mathcal{I}\}}$, where $y_{ui}=1$ indicates method $u$ has called API $i$, otherwise $y_{ui}=0$.

\noindent\textbf{API Global Co-occurrence Graph:} In addition to call interaction, there are also co-occurrence relations between APIs, for example, \emph{file.open()} and \emph{file.close()} often appear together. We consider all APIs called by corresponding method as an API sequence. For k-th API ${i_k^s}$ in sequence ${S}$, the neighbor set of ${i_k^s}$ indicates a set of APIs, each element of which is defined as follows: ${\mathcal{N}({i_k^s}) = \{i_n^s|i_n^s\in{S};n\in[k,k+\varepsilon]\}}$, ${\varepsilon}$ is window size to control the scope of modeling of API-connection between ${i_k^s}$ and ${i_n^s}$. Note that, the hyperparameter ${\varepsilon}$ favors the modeling of short-range links since it is helpless (even noise, e.g., irrelevant dependence) for capturing the whole sequence length information if beyond the scope ${\varepsilon}$. Based on neighbor sets of APIs in all sequences, we build the API global co-occurrence graph $\mathcal{G}_O$. Since APIs often appear together several times, we consider frequency ${\mathcal{T}}$ as the edge type of $\mathcal{G}_O$. Formally, the graph is presented as $\{(i,f,j)|i,j\in\mathcal{I},f\in\mathcal{T}\}$, where each triplet describes that API $i$ and API $j$ are invocated together in a method $f$ times. For example, $(file.open(),10 ,file.close())$ states that file.open() and file.close() appear together 10 times.

\noindent\textbf{Method/API Hierarchical Relation Graph:} In addition to invocation information and co-occurrence information, method and API have abundant structural information in software projects. For example, the tree structure of project contains hierarchical relation information: a project consists of a number of classes, and a class consists of a number of methods. We organize the side information in the form of directed graph $\mathcal{G}_H=\{(h,r,t)|h,t\in\mathcal{E},r\in\mathcal{R}\}$, in which each triple $(h,r,t)$ denotes that there is a relation $r$ from head entity $h$ to tail entity $t$. To be specific, $\mathcal{E}$ contains all methods, APIs, classes and projects and $\mathcal{R}$ contains two type of relationship, i.e., belong-to-class, belong-to-project. For example, \emph{(getById, belong-to-class, CustomerDAO)} states the fact that method \emph{getById} belongs to class \emph{CustomerDAO}.
 
 
\noindent\textbf{Task Description:} Given call interaction graph ${\mathcal{G}_I}$, API global co-occurrence graph ${\mathcal{G}_O}$ and method/API hierarchical relation graph ${\mathcal{G}_H}$, the task is to predict the probability that method $u$ will invocate API $i$. 
Specifically, our goal is to learn a prediction function $\hat{y}_{ui}=\mathcal{F}(u,i|\Theta)$, where $\hat{y}_{ui}$ denotes the predicted probability and $\Theta$ denotes the model parameters of function $\mathcal{F}$.

\begin{figure}
  \centering
  \includegraphics[scale=0.25]{figures/method-OverallWorkflow.pdf}
  \caption{The Overall Workflow of \tool}
  \label{fig:workflow}
  \Description{model}
\end{figure}
